RLSbench: Domain Adaptation Under Relaxed Label Shift

Despite the emergence of principled methods for domain adaptation under label shift, their sensitivity to shifts in class conditional distributions is precariously under explored. Meanwhile, popular deep domain adaptation heuristics tend to falter when faced with label proportions shifts. While several papers modify these heuristics in attempts to handle label proportions shifts, inconsistencies in evaluation standards, datasets, and baselines make it difficult to gauge the current best practices. In this paper, we introduce RLSbench, a large-scale benchmark for relaxed label shift, consisting of $>$500 distribution shift pairs spanning vision, tabular, and language modalities, with varying label proportions. Unlike existing benchmarks, which primarily focus on shifts in class-conditional $p(x|y)$, our benchmark also focuses on label marginal shifts. First, we assess 13 popular domain adaptation methods, demonstrating more widespread failures under label proportion shifts than were previously known. Next, we develop an effective two-step meta-algorithm that is compatible with most domain adaptation heuristics: (i) pseudo-balance the data at each epoch; and (ii) adjust the final classifier with target label distribution estimate. The meta-algorithm improves existing domain adaptation heuristics under large label proportion shifts, often by 2--10\% accuracy points, while conferring minimal effect ($<$0.5\%) when label proportions do not shift. We hope that these findings and the availability of RLSbench will encourage researchers to rigorously evaluate proposed methods in relaxed label shift settings. Code is publicly available at https://github.com/acmi-lab/RLSbench.

==> sections/exp_outline.tex <==





==> sections/future_work.tex <==


    
    



==> tables/camelyon.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
Source (w/o aug) &    &          81.8 &  81.8 &  81.9 &    &         82.2 &  82.3 &  82.3 &    &        82.4 &  82.6 &  82.6 &    &        79.6 &  81.7 &  85.0 &    &        79.8 &  81.4 &  84.0 \\
  Source (w aug) &    &          78.0 &  77.1 &  78.0 &    &         79.4 &  78.7 &  79.3 &    &        80.5 &  80.0 &  80.5 &    &        68.6 &  67.4 &  74.3 &    &        69.5 &  68.4 &  74.0 \\
    Source (adv) &    &          82.8 &  82.1 &  82.8 &    &         83.4 &  82.8 &  83.2 &    &        84.0 &  83.5 &  83.8 &    &        77.8 &  79.0 &  85.2 &    &        78.3 &  79.2 &  84.2 \\
   Source (clip) &    &          96.1 &  96.1 &  96.1 &    &         96.3 &  96.3 &  96.3 &    &        96.5 &  96.4 &  96.4 &    &        94.8 &  95.3 &  95.5 &    &        94.9 &  95.3 &  95.5 \\
            DARE &    &          79.0 &  79.0 &  79.1 &    &         79.5 &  79.5 &  79.5 &    &        79.7 &  79.8 &  79.9 &    &        73.9 &  74.2 &  76.9 &    &        74.4 &  74.8 &  76.9 \\
        BN-adapt &    &          89.5 &  88.7 &  89.4 &    &         89.0 &  88.6 &  89.2 &    &        85.8 &  85.2 &  86.5 &    &        84.3 &  90.1 &  88.7 &    &        84.6 &  87.8 &  89.1 \\
     RS-BN-adapt &    &          88.6 &  87.3 &  88.6 &    &         88.8 &  88.2 &  89.1 &    &        87.6 &  87.0 &  88.3 &    &        89.0 &  90.3 &  92.1 &    &        90.0 &  87.6 &  92.4 \\
            TENT &    &          92.3 &  92.1 &  92.3 &    &         90.3 &  90.4 &  90.5 &    &        91.0 &  90.9 &  91.3 &    &        81.9 &  85.6 &  85.0 &    &        81.1 &  83.4 &  84.5 \\
         RS-TENT &    &          92.0 &  90.4 &  92.0 &    &         92.7 &  92.7 &  92.9 &    &        90.9 &  90.9 &  91.2 &    &        85.1 &  90.3 &  89.6 &    &        86.6 &  87.6 &  89.7 \\
            DANN &    &          83.0 &  82.7 &  83.1 &    &         84.2 &  83.9 &  84.2 &    &        85.2 &  85.1 &  85.3 &    &        75.2 &  74.6 &  79.0 &    &        78.2 &  78.3 &  80.7 \\
         IW-DANN &    &          84.1 &       &       &    &         84.2 &       &       &    &        85.9 &       &       &    &        78.7 &       &       &    &        78.1 &       &       \\
         RS-DANN &    &          84.1 &  83.7 &  84.1 &    &         83.7 &  82.9 &  83.5 &    &        86.5 &  86.2 &  86.5 &    &        71.6 &  70.8 &  75.0 &    &        75.9 &  75.7 &  78.4 \\
           CDANN &    &          87.3 &  87.1 &  87.3 &    &         87.3 &  87.0 &  87.4 &    &        87.0 &  87.0 &  87.1 &    &        80.7 &  81.4 &  86.8 &    &        79.7 &  79.8 &  83.3 \\
        IW-CDANN &    &          87.2 &       &       &    &         85.3 &       &       &    &        85.5 &       &       &    &        81.6 &       &       &    &        86.1 &       &       \\
        RS-CDANN &    &          88.1 &  87.8 &  88.1 &    &         83.2 &  83.2 &  83.3 &    &        85.8 &  85.8 &  86.0 &    &        88.7 &  90.5 &  91.3 &    &        92.2 &  93.3 &  93.4 \\
        FixMatch &    &          91.3 &  91.3 &  91.3 &    &         92.7 &  92.5 &  92.5 &    &        93.6 &  93.8 &  93.7 &    &        79.9 &  82.1 &  83.8 &    &        81.5 &  82.7 &  84.0 \\
     RS-FixMatch &    &          88.6 &  87.8 &  88.6 &    &         93.7 &  93.5 &  93.6 &    &        94.2 &  94.2 &  94.2 &    &        81.5 &  82.9 &  84.2 &    &        80.1 &  80.6 &  82.8 \\
    NoisyStudent &    &          88.4 &  88.1 &  88.4 &    &         85.9 &  84.9 &  85.9 &    &        88.2 &  87.9 &  88.3 &    &        83.0 &  83.7 &  86.1 &    &        84.4 &  85.4 &  86.8 \\
 RS-NoisyStudent &    &          87.7 &  87.1 &  87.7 &    &         85.7 &  84.7 &  85.6 &    &        88.6 &  88.2 &  88.8 &    &        84.9 &  85.9 &  87.6 &    &        85.3 &  86.1 &  87.5 \\
          SENTRY &    &          90.7 &  90.4 &  90.7 &    &         91.5 &  91.2 &  91.4 &    &        90.6 &  90.7 &  90.7 &    &        80.7 &  81.9 &  82.4 &    &        83.5 &  84.9 &  85.0 \\
\bottomrule
\end{tabular}

==> tables/cifar10.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
Source (w/o aug) &    &          87.6 &  87.3 &  87.6 &    &         87.2 &  86.9 &  87.5 &    &        87.3 &  87.2 &  88.0 &    &        88.1 &  90.4 &  91.1 &    &        91.0 &  93.6 &  94.0 \\
  Source (w aug) &    &          89.9 &  89.7 &  89.9 &    &         90.0 &  89.5 &  89.8 &    &        90.1 &  90.0 &  90.4 &    &        90.6 &  92.4 &  92.7 &    &        92.9 &  95.0 &  95.3 \\
    Source (adv) &    &          59.8 &  33.2 &  59.8 &    &         61.8 &  34.8 &  55.1 &    &        64.2 &  38.1 &  54.0 &    &        56.1 &  42.2 &  67.4 &    &        54.9 &  51.9 &  68.7 \\
   Source (clip) &    &          89.3 &  88.5 &  89.3 &    &         89.1 &  88.4 &  89.5 &    &        89.1 &  88.7 &  90.0 &    &        89.2 &  88.9 &  90.0 &    &        88.8 &  88.9 &  91.5 \\
            DARE &    &          85.0 &  84.9 &  85.0 &    &         83.1 &  83.4 &  83.4 &    &        80.5 &  80.9 &  81.2 &    &        72.4 &  73.1 &  74.4 &    &        61.1 &  62.8 &  70.7 \\
        BN-adapt &    &          90.4 &  90.2 &  90.4 &    &         89.3 &  89.5 &  89.7 &    &        87.9 &  89.5 &  89.9 &    &        85.4 &  89.8 &  91.1 &    &        80.3 &  89.9 &  93.1 \\
     RS-BN-adapt &    &          90.5 &  90.3 &  90.5 &    &         90.3 &  90.2 &  90.6 &    &        90.5 &  90.5 &  91.1 &    &        91.1 &  92.8 &  93.0 &    &        91.2 &  95.4 &  96.0 \\
            TENT &    &          90.7 &  90.4 &  90.7 &    &         89.4 &  89.6 &  89.9 &    &        87.9 &  89.5 &  89.8 &    &        85.6 &  90.1 &  91.3 &    &        80.1 &  90.1 &  93.1 \\
         RS-TENT &    &          90.5 &  90.4 &  90.5 &    &         90.3 &  90.2 &  90.6 &    &        90.4 &  90.4 &  91.0 &    &        91.1 &  92.8 &  93.0 &    &        91.2 &  95.4 &  95.9 \\
            DANN &    &          86.6 &  86.0 &  86.6 &    &         86.3 &  86.0 &  86.6 &    &        86.0 &  86.2 &  86.6 &    &        86.0 &  89.5 &  90.3 &    &        90.0 &  93.3 &  93.8 \\
         IW-DANN &    &          86.6 &       &       &    &         86.4 &       &       &    &        86.2 &       &       &    &        85.9 &       &       &    &        89.8 &       &       \\
         RS-DANN &    &          85.1 &  83.2 &  85.1 &    &         84.7 &  83.0 &  84.6 &    &        84.3 &  83.1 &  84.3 &    &        85.2 &  87.0 &  88.2 &    &        88.9 &  91.4 &  91.7 \\
           CDANN &    &          86.5 &  86.0 &  86.5 &    &         86.0 &  85.6 &  86.3 &    &        85.8 &  85.7 &  86.4 &    &        85.8 &  89.7 &  90.5 &    &        90.0 &  93.3 &  93.6 \\
        IW-CDANN &    &          86.5 &       &       &    &         86.0 &       &       &    &        85.8 &       &       &    &        85.9 &       &       &    &        90.0 &       &       \\
        RS-CDANN &    &          86.6 &  86.0 &  86.6 &    &         86.4 &  85.8 &  86.6 &    &        85.7 &  85.5 &  86.4 &    &        86.6 &  90.2 &  90.5 &    &        90.3 &  93.3 &  93.7 \\
        FixMatch &    &          91.0 &  90.9 &  91.0 &    &         91.2 &  91.2 &  91.3 &    &        91.3 &  91.4 &  91.8 &    &        91.1 &  93.4 &  93.5 &    &        91.3 &  95.1 &  95.8 \\
     RS-FixMatch &    &          91.4 &  91.2 &  91.4 &    &         91.6 &  91.4 &  91.6 &    &        91.5 &  91.8 &  91.9 &    &        92.0 &  93.4 &  93.6 &    &        94.2 &  95.7 &  95.9 \\
    NoisyStudent &    &          91.0 &  90.8 &  91.0 &    &         91.1 &  90.5 &  90.8 &    &        91.1 &  91.0 &  91.2 &    &        92.6 &  93.8 &  93.9 &    &        95.0 &  95.6 &  95.7 \\
 RS-NoisyStudent &    &          91.0 &  90.8 &  91.0 &    &         91.1 &  90.5 &  90.8 &    &        91.1 &  91.0 &  91.2 &    &        92.6 &  93.8 &  93.9 &    &        95.0 &  95.6 &  95.7 \\
          SENTRY &    &          88.6 &  88.3 &  88.6 &    &         88.4 &  88.4 &  88.7 &    &        88.4 &  88.6 &  88.9 &    &        88.8 &  91.3 &  91.9 &    &        89.1 &  93.9 &  94.4 \\
\bottomrule
\end{tabular}


==> tables/cifar100.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
 Source (w/o aug) &    &          64.1 &  58.0 &  64.1 &    &         65.6 &  59.1 &  65.3 &    &        64.7 &  58.1 &  66.0 &    &        64.4 &  62.1 &  72.6 &    &        66.6 &  69.3 &  79.2 \\
   Source (w aug) &    &          70.2 &  66.7 &  70.2 &    &         71.5 &  67.3 &  71.8 &    &        70.2 &  65.7 &  72.3 &    &        69.8 &  70.2 &  77.2 &    &        71.5 &  76.2 &  82.4 \\
     Source (adv) &    &          26.1 &  18.6 &  26.1 &    &         26.2 &  19.5 &  27.3 &    &        25.5 &  19.2 &  28.6 &    &        25.0 &  19.7 &  34.8 &    &        28.2 &  28.5 &  43.0 \\
    Source (clip) &    &          83.0 &  82.6 &  83.0 &    &         84.2 &  83.8 &  84.4 &    &        84.4 &  84.1 &  85.0 &    &        83.9 &  86.1 &  88.0 &    &        85.2 &  87.1 &  91.6 \\
             DARE &    &          64.1 &  63.9 &  64.1 &    &         63.4 &  63.2 &  63.7 &    &        59.0 &  58.1 &  59.4 &    &        46.5 &  46.5 &  53.6 &    &        37.4 &  38.6 &  58.3 \\
         BN-adapt &    &          71.6 &  69.4 &  71.6 &    &         72.9 &  69.8 &  73.0 &    &        71.0 &  67.9 &  73.2 &    &        70.5 &  73.1 &  78.4 &    &        71.6 &  78.1 &  82.4 \\
      RS-BN-adapt &    &          71.5 &  69.2 &  71.5 &    &         72.6 &  69.7 &  72.9 &    &        71.3 &  68.1 &  73.1 &    &        71.1 &  72.8 &  78.1 &    &        72.9 &  78.3 &  82.5 \\
             TENT &    &          71.4 &  69.4 &  71.4 &    &         72.6 &  69.8 &  73.0 &    &        71.0 &  68.0 &  73.0 &    &        70.4 &  72.9 &  77.9 &    &        71.9 &  78.0 &  82.5 \\
          RS-TENT &    &          71.5 &  69.2 &  71.5 &    &         72.4 &  69.5 &  72.7 &    &        71.3 &  68.2 &  73.0 &    &        71.4 &  72.7 &  78.1 &    &        73.0 &  78.3 &  82.5 \\
             DANN &    &          78.3 &  77.8 &  78.3 &    &         78.7 &  78.5 &  79.0 &    &        77.9 &  77.4 &  79.0 &    &        75.7 &  79.9 &  82.0 &    &        78.7 &  83.4 &  86.1 \\
          IW-DANN &    &          78.3 &       &       &    &         79.0 &       &       &    &        77.7 &       &       &    &        77.4 &       &       &    &        80.0 &       &       \\
          RS-DANN &    &          78.3 &  77.7 &  78.3 &    &         78.3 &  77.4 &  78.4 &    &        76.8 &  76.2 &  78.2 &    &        75.4 &  78.5 &  81.1 &    &        74.3 &  77.8 &  81.8 \\
            CDANN &    &          77.9 &  77.3 &  77.9 &    &         77.9 &  77.6 &  78.3 &    &        75.9 &  75.6 &  77.0 &    &        75.7 &  78.2 &  80.5 &    &        79.4 &  82.3 &  86.4 \\
         IW-CDANN &    &          77.7 &       &       &    &         77.6 &       &       &    &        76.4 &       &       &    &        77.1 &       &       &    &        79.3 &       &       \\
         RS-CDANN &    &          77.4 &  76.9 &  77.4 &    &         78.0 &  77.4 &  78.1 &    &        77.0 &  76.3 &  77.8 &    &        76.4 &  78.4 &  81.1 &    &        77.2 &  80.2 &  85.2 \\
         FixMatch &    &          72.1 &  69.5 &  72.1 &    &         72.1 &  69.2 &  72.5 &    &        70.7 &  67.8 &  72.8 &    &        71.1 &  71.9 &  77.6 &    &        74.1 &  77.9 &  81.4 \\
      RS-FixMatch &    &          71.9 &  69.6 &  71.9 &    &         72.6 &  70.2 &  73.3 &    &        71.1 &  68.4 &  73.0 &    &        71.6 &  73.1 &  78.1 &    &        73.6 &  77.1 &  81.6 \\
     NoisyStudent &    &          71.3 &  68.4 &  71.3 &    &         71.7 &  68.8 &  72.3 &    &        70.4 &  66.9 &  71.3 &    &        72.1 &  72.8 &  77.0 &    &        73.9 &  78.0 &  80.8 \\
  RS-NoisyStudent &    &          71.3 &  68.3 &  71.3 &    &         71.6 &  68.9 &  72.3 &    &        70.3 &  66.7 &  71.0 &    &        72.4 &  73.0 &  77.2 &    &        73.8 &  78.0 &  80.9 \\
           SENTRY &    &          67.6 &  64.0 &  67.6 &    &         68.3 &  64.7 &  68.9 &    &        67.3 &  63.0 &  69.2 &    &        68.9 &  70.0 &  74.9 &    &        69.6 &  73.0 &  78.6 \\
 \bottomrule
 \end{tabular}
 

==> tables/domainnet.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
Source (w/o aug) &    &          49.4 &  45.1 &  51.0 &    &         49.4 &  45.5 &  51.8 &    &        49.0 &  45.7 &  52.5 &    &        50.1 &  47.7 &  56.5 &    &        48.6 &  48.4 &  59.0 \\
  Source (w aug) &    &          53.0 &  49.2 &  54.6 &    &         53.0 &  49.6 &  55.2 &    &        52.5 &  49.7 &  56.1 &    &        53.1 &  51.6 &  60.4 &    &        52.8 &  52.8 &  61.9 \\
    Source (adv) &    &          48.7 &  43.5 &  50.5 &    &         48.8 &  43.6 &  51.2 &    &        48.6 &  44.2 &  52.3 &    &        49.5 &  46.8 &  56.0 &    &        49.0 &  47.3 &  58.4 \\
   Source (clip) &    &          70.8 &  68.8 &  72.2 &    &         71.4 &  69.4 &  73.6 &    &        71.2 &  69.5 &  73.9 &    &        71.4 &  70.9 &  76.3 &    &        71.7 &  72.0 &  79.1 \\
            DARE &    &          51.5 &  51.1 &  53.0 &    &         50.4 &  49.9 &  52.6 &    &        48.3 &  48.0 &  52.2 &    &        45.8 &  45.7 &  53.8 &    &        38.3 &  39.3 &  51.5 \\
        BN-adapt &    &          53.7 &  52.7 &  55.6 &    &         53.6 &  52.5 &  56.6 &    &        53.3 &  52.7 &  57.4 &    &        54.4 &  54.2 &  61.4 &    &        52.2 &  54.7 &  62.5 \\
     RS-BN-adapt &    &          54.1 &  52.7 &  55.9 &    &         53.9 &  52.9 &  56.6 &    &        53.2 &  52.6 &  57.2 &    &        54.5 &  54.1 &  62.1 &    &        52.4 &  54.5 &  62.6 \\
            TENT &    &          55.3 &  54.4 &  57.0 &    &         54.2 &  53.3 &  57.2 &    &        54.0 &  53.5 &  58.2 &    &        54.5 &  54.6 &  61.5 &    &        52.4 &  55.2 &  62.8 \\
         RS-TENT &    &          55.8 &  55.1 &  57.6 &    &         54.7 &  53.7 &  57.3 &    &        53.9 &  53.2 &  58.1 &    &        54.6 &  54.2 &  61.9 &    &        52.9 &  55.0 &  63.0 \\
            DANN &    &          53.8 &  53.1 &  55.8 &    &         53.5 &  53.0 &  56.7 &    &        52.1 &  51.6 &  56.3 &    &        52.4 &  52.2 &  59.4 &    &        47.3 &  49.3 &  59.6 \\
         IW-DANN &    &          54.2 &       &       &    &         53.7 &       &       &    &        52.7 &       &       &    &        51.3 &       &       &    &        48.4 &       &       \\
         RS-DANN &    &          55.1 &  54.3 &  56.4 &    &         54.9 &  54.3 &  57.2 &    &        54.1 &  53.4 &  56.9 &    &        52.2 &  52.2 &  59.0 &    &        51.0 &  52.0 &  60.1 \\
           CDANN &    &          55.7 &  54.8 &  57.1 &    &         54.6 &  53.5 &  57.2 &    &        54.1 &  53.1 &  57.2 &    &        53.4 &  53.0 &  60.4 &    &        52.2 &  54.2 &  60.5 \\
        IW-CDANN &    &          55.9 &       &       &    &         55.0 &       &       &    &        54.4 &       &       &    &        53.8 &       &       &    &        51.6 &       &       \\
        RS-CDANN &    &          56.2 &  55.3 &  57.5 &    &         55.5 &  54.4 &  57.8 &    &        54.7 &  53.9 &  57.7 &    &        54.1 &  53.8 &  60.7 &    &        53.4 &  54.0 &  62.0 \\
        FixMatch &    &          57.6 &  55.7 &  59.0 &    &         57.6 &  55.8 &  59.6 &    &        57.6 &  55.8 &  60.0 &    &        58.4 &  57.4 &  63.1 &    &        58.4 &  58.8 &  63.8 \\
     RS-FixMatch &    &          58.6 &  56.6 &  59.1 &    &         58.0 &  56.2 &  59.4 &    &        57.7 &  56.0 &  59.5 &    &        59.1 &  58.3 &  63.2 &    &        58.6 &  58.8 &  64.4 \\
    NoisyStudent &    &          54.9 &  52.0 &  56.1 &    &         53.7 &  50.8 &  55.8 &    &        53.5 &  51.1 &  56.2 &    &        54.1 &  52.8 &  60.2 &    &        55.5 &  55.2 &  63.1 \\
 RS-NoisyStudent &    &          54.6 &  51.3 &  55.8 &    &         53.5 &  50.6 &  55.3 &    &        53.6 &  50.7 &  56.3 &    &        54.9 &  52.9 &  60.4 &    &        54.9 &  54.9 &  62.7 \\
          SENTRY &    &          57.3 &  56.0 &  57.4 &    &         49.0 &  45.2 &  50.1 &    &        51.6 &  49.0 &  53.6 &    &        48.3 &  46.0 &  53.7 &    &        46.3 &  44.9 &  53.7 \\
\bottomrule
\end{tabular}

==> tables/entity13.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
 Source (w/o aug) &    &          73.4 &  73.1 &  73.4 &    &         74.3 &  74.2 &  74.7 &    &        76.8 &  77.5 &  78.4 &    &        80.0 &  81.1 &  83.8 &    &        78.6 &  80.3 &  83.8 \\
   Source (w aug) &    &          78.2 &  78.3 &  78.2 &    &         80.2 &  79.9 &  80.1 &    &        82.3 &  82.5 &  83.1 &    &        85.3 &  86.3 &  87.1 &    &        81.5 &  85.0 &  86.1 \\
     Source (adv) &    &          73.2 &  71.5 &  73.2 &    &         75.5 &  74.5 &  75.5 &    &        78.3 &  76.6 &  78.2 &    &        79.7 &  80.8 &  83.2 &    &        76.9 &  81.8 &  83.4 \\
    Source (clip) &    &          88.8 &  88.9 &  88.8 &    &         89.8 &  90.1 &  90.1 &    &        90.3 &  90.5 &  90.6 &    &        92.4 &  92.7 &  94.4 &    &        91.5 &  92.4 &  94.1 \\
             DARE &    &          73.9 &  74.0 &  73.9 &    &         73.5 &  73.5 &  73.9 &    &        72.4 &  72.1 &  72.7 &    &        63.9 &  64.3 &  72.8 &    &        55.5 &  57.2 &  64.7 \\
         BN-adapt &    &          77.9 &  77.8 &  77.9 &    &         79.8 &  79.7 &  79.7 &    &        81.3 &  81.7 &  82.4 &    &        82.4 &  84.4 &  85.9 &    &        76.1 &  80.0 &  83.2 \\
      RS-BN-adapt &    &          77.5 &  77.4 &  77.5 &    &         79.8 &  79.6 &  79.6 &    &        82.0 &  82.4 &  82.5 &    &        84.9 &  86.1 &  86.7 &    &        80.6 &  84.0 &  86.3 \\
             TENT &    &          77.9 &  77.8 &  77.9 &    &         79.9 &  79.7 &  79.8 &    &        81.4 &  81.8 &  82.5 &    &        82.5 &  84.5 &  86.0 &    &        76.2 &  80.1 &  83.2 \\
          RS-TENT &    &          77.5 &  77.5 &  77.5 &    &         79.9 &  79.6 &  79.7 &    &        82.1 &  82.4 &  82.5 &    &        84.9 &  86.1 &  86.7 &    &        80.6 &  84.0 &  86.3 \\
             DANN &    &          75.7 &  75.3 &  75.7 &    &         77.4 &  77.5 &  77.9 &    &        79.1 &  80.2 &  80.6 &    &        80.7 &  83.4 &  84.7 &    &        79.3 &  80.9 &  82.1 \\
          IW-DANN &    &          76.0 &       &       &    &         77.5 &       &       &    &        79.8 &       &       &    &        83.5 &       &       &    &        77.9 &       &       \\
          RS-DANN &    &          75.5 &  75.3 &  75.5 &    &         77.1 &  77.8 &  77.9 &    &        79.8 &  80.5 &  80.5 &    &        82.9 &  85.1 &  85.7 &    &        77.9 &  80.4 &  81.9 \\
            CDANN &    &          76.2 &  75.9 &  76.2 &    &         77.5 &  77.8 &  78.8 &    &        78.7 &  79.7 &  80.5 &    &        82.4 &  86.0 &  87.2 &    &        77.7 &  81.6 &  83.3 \\
         IW-CDANN &    &          75.4 &       &       &    &         77.2 &       &       &    &        78.5 &       &       &    &        83.3 &       &       &    &        79.2 &       &       \\
         RS-CDANN &    &          74.1 &  73.6 &  74.1 &    &         77.8 &  78.3 &  78.2 &    &        79.7 &  80.1 &  80.7 &    &        81.4 &  85.1 &  86.3 &    &        73.8 &  77.1 &  78.8 \\
         FixMatch &    &          79.8 &  79.9 &  79.8 &    &         80.4 &  80.4 &  80.9 &    &        81.9 &  82.4 &  82.9 &    &        82.2 &  85.5 &  88.2 &    &        76.6 &  79.6 &  81.2 \\
      RS-FixMatch &    &          80.5 &  80.4 &  80.5 &    &         81.0 &  81.4 &  81.6 &    &        82.6 &  83.1 &  83.8 &    &        87.5 &  88.1 &  89.2 &    &        79.9 &  83.5 &  85.4 \\
     NoisyStudent &    &          78.9 &  78.5 &  78.9 &    &         78.4 &  78.5 &  78.8 &    &        80.9 &  81.5 &  81.8 &    &        85.2 &  86.5 &  88.2 &    &        82.8 &  85.7 &  88.0 \\
  RS-NoisyStudent &    &          79.0 &  78.8 &  79.0 &    &         80.7 &  80.9 &  80.8 &    &        80.3 &  81.2 &  81.9 &    &        84.7 &  87.8 &  89.0 &    &        83.2 &  85.2 &  86.6 \\
           SENTRY &    &          76.6 &  76.4 &  76.6 &    &         76.3 &  74.8 &  76.8 &    &        69.9 &  67.7 &  70.6 &    &        80.7 &  82.0 &  83.3 &    &        56.5 &  57.6 &  60.9 \\
 \bottomrule
 \end{tabular}
 

==> tables/entity30.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
Source (w/o aug) &    &          63.5 &  63.1 &  63.5 &    &         62.9 &  63.4 &  63.6 &    &        63.4 &  64.6 &  65.1 &    &        64.4 &  67.9 &  74.7 &    &        56.0 &  63.5 &  78.4 \\
  Source (w aug) &    &          70.2 &  69.8 &  70.2 &    &         71.2 &  70.5 &  70.9 &    &        70.6 &  70.1 &  71.4 &    &        72.4 &  73.8 &  75.7 &    &        64.8 &  70.5 &  81.3 \\
    Source (adv) &    &          61.2 &  59.7 &  61.2 &    &         61.6 &  60.8 &  62.9 &    &        62.3 &  61.5 &  65.2 &    &        64.3 &  66.5 &  70.3 &    &        55.3 &  59.3 &  77.0 \\
   Source (clip) &    &          85.3 &  85.0 &  85.3 &    &         85.8 &  85.3 &  85.8 &    &        85.4 &  85.4 &  85.9 &    &        85.8 &  87.9 &  89.2 &    &        81.3 &  83.5 &  89.2 \\
            DARE &    &          66.7 &  66.4 &  66.7 &    &         65.3 &  65.7 &  65.2 &    &        62.2 &  62.4 &  63.4 &    &        50.8 &  50.4 &  57.5 &    &        27.3 &  28.4 &  53.6 \\
        BN-adapt &    &          69.9 &  69.6 &  69.9 &    &         70.2 &  70.0 &  70.6 &    &        69.4 &  70.0 &  71.0 &    &        71.2 &  73.1 &  74.7 &    &        61.6 &  67.5 &  80.0 \\
     RS-BN-adapt &    &          70.0 &  69.6 &  70.0 &    &         70.8 &  70.7 &  71.3 &    &        69.7 &  70.8 &  71.8 &    &        72.1 &  73.8 &  75.3 &    &        63.9 &  69.8 &  80.8 \\
            TENT &    &          69.9 &  69.7 &  69.9 &    &         70.3 &  70.0 &  70.6 &    &        69.4 &  70.0 &  71.0 &    &        71.2 &  73.1 &  74.7 &    &        61.7 &  67.5 &  80.0 \\
         RS-TENT &    &          70.1 &  69.7 &  70.1 &    &         70.8 &  70.5 &  71.5 &    &        69.8 &  70.8 &  71.9 &    &        72.1 &  73.8 &  75.3 &    &        63.9 &  69.8 &  80.8 \\
            DANN &    &          67.3 &  67.0 &  67.3 &    &         67.5 &  67.1 &  67.5 &    &        66.2 &  66.6 &  68.8 &    &        66.9 &  68.6 &  75.3 &    &        61.0 &  65.4 &  80.3 \\
         IW-DANN &    &          66.1 &       &       &    &         66.3 &       &       &    &        67.1 &       &       &    &        70.6 &       &       &    &        60.2 &       &       \\
         RS-DANN &    &          66.5 &  66.5 &  66.5 &    &         67.8 &  67.7 &  68.7 &    &        67.0 &  66.4 &  68.8 &    &        70.2 &  71.9 &  77.1 &    &        55.3 &  62.2 &  79.4 \\
           CDANN &    &          65.8 &  66.1 &  65.8 &    &         66.8 &  65.9 &  66.6 &    &        66.8 &  66.1 &  68.9 &    &        69.0 &  70.9 &  74.9 &    &        55.4 &  61.6 &  76.8 \\
        IW-CDANN &    &          67.8 &       &       &    &         66.2 &       &       &    &        65.7 &       &       &    &        70.0 &       &       &    &        53.4 &       &       \\
        RS-CDANN &    &          66.0 &  66.1 &  66.0 &    &         68.4 &  68.2 &  67.4 &    &        67.5 &  69.1 &  70.2 &    &        69.7 &  72.4 &  76.9 &    &        61.5 &  66.9 &  78.1 \\
        FixMatch &    &          72.3 &  71.6 &  72.3 &    &         72.9 &  73.2 &  73.5 &    &        73.9 &  74.1 &  74.4 &    &        74.4 &  76.1 &  78.3 &    &        64.0 &  68.5 &  78.5 \\
     RS-FixMatch &    &          73.4 &  72.7 &  73.4 &    &         72.2 &  71.5 &  71.9 &    &        71.3 &  72.4 &  73.6 &    &        70.4 &  72.9 &  77.5 &    &        60.4 &  68.4 &  79.4 \\
    NoisyStudent &    &          70.5 &  69.4 &  70.5 &    &         70.0 &  69.8 &  70.5 &    &        71.7 &  71.0 &  72.2 &    &        72.9 &  74.2 &  76.7 &    &        63.6 &  65.8 &  76.0 \\
 RS-NoisyStudent &    &          70.3 &  70.2 &  70.3 &    &         71.6 &  71.4 &  71.5 &    &        71.4 &  71.2 &  71.3 &    &        72.7 &  74.3 &  77.7 &    &        60.9 &  66.5 &  81.2 \\
          SENTRY &    &          64.4 &  62.5 &  64.4 &    &         64.8 &  63.8 &  64.4 &    &        62.3 &  61.4 &  63.2 &    &        54.1 &  55.2 &  60.4 &    &        39.3 &  41.6 &  71.4 \\
\bottomrule
\end{tabular}

==> tables/fmow.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
 Source (w/o aug) &    &          56.4 &  55.7 &  56.5 &    &         57.7 &  57.2 &  57.8 &    &        57.6 &  58.2 &  58.7 &    &        59.7 &  62.1 &  64.1 &    &        55.7 &  59.1 &  61.9 \\
   Source (w aug) &    &          59.7 &  57.9 &  59.8 &    &         60.5 &  58.9 &  60.9 &    &        60.1 &  59.9 &  62.1 &    &        61.7 &  64.5 &  67.9 &    &        58.6 &  63.3 &  67.5 \\
     Source (adv) &    &          48.4 &  44.0 &  48.6 &    &         49.3 &  45.2 &  49.8 &    &        49.7 &  45.7 &  51.4 &    &        51.5 &  50.2 &  57.9 &    &        48.7 &  50.6 &  57.0 \\
    Source (clip) &    &          64.0 &  63.2 &  64.1 &    &         65.1 &  64.2 &  65.4 &    &        65.3 &  65.3 &  66.9 &    &        66.3 &  68.2 &  71.6 &    &        61.8 &  66.4 &  69.9 \\
             DARE &    &          53.9 &  53.6 &  54.0 &    &         54.0 &  54.1 &  54.4 &    &        51.7 &  51.5 &  52.6 &    &        45.7 &  46.7 &  52.1 &    &        41.5 &  41.8 &  50.3 \\
         BN-adapt &    &          57.1 &  55.7 &  57.3 &    &         57.6 &  56.3 &  58.0 &    &        56.9 &  56.1 &  58.8 &    &        58.5 &  60.7 &  64.8 &    &        53.7 &  58.7 &  62.9 \\
      RS-BN-adapt &    &          56.8 &  55.5 &  57.0 &    &         57.2 &  55.3 &  57.7 &    &        56.7 &  55.5 &  58.5 &    &        60.0 &  60.9 &  65.2 &    &        55.0 &  59.0 &  64.0 \\
             TENT &    &          57.2 &  54.5 &  57.4 &    &         58.7 &  57.5 &  59.0 &    &        58.9 &  57.7 &  60.4 &    &        59.6 &  61.0 &  64.4 &    &        55.8 &  60.2 &  63.9 \\
          RS-TENT &    &          58.0 &  55.0 &  58.1 &    &         59.1 &  57.7 &  59.6 &    &        57.6 &  56.0 &  59.2 &    &        59.5 &  61.3 &  64.6 &    &        55.0 &  59.0 &  63.7 \\
             DANN &    &          57.2 &  55.8 &  57.3 &    &         59.1 &  57.7 &  59.1 &    &        57.8 &  56.8 &  59.2 &    &        59.5 &  60.2 &  64.6 &    &        55.3 &  59.3 &  63.0 \\
          IW-DANN &    &          57.1 &       &       &    &         58.7 &       &       &    &        58.1 &       &       &    &        56.3 &       &       &    &        55.2 &       &       \\
          RS-DANN &    &          56.6 &  55.1 &  56.8 &    &         57.2 &  55.6 &  57.6 &    &        57.2 &  56.5 &  58.9 &    &        59.2 &  59.4 &  63.0 &    &        53.9 &  57.9 &  60.9 \\
            CDANN &    &          57.3 &  55.9 &  57.4 &    &         58.3 &  56.7 &  58.5 &    &        58.2 &  56.7 &  59.8 &    &        58.2 &  59.0 &  63.8 &    &        54.9 &  57.5 &  62.4 \\
         IW-CDANN &    &          57.2 &       &       &    &         58.1 &       &       &    &        57.9 &       &       &    &        59.3 &       &       &    &        53.3 &       &       \\
         RS-CDANN &    &          56.3 &  55.4 &  56.5 &    &         57.3 &  56.6 &  57.7 &    &        56.2 &  54.8 &  58.0 &    &        56.3 &  57.5 &  61.3 &    &        54.6 &  56.8 &  60.6 \\
         FixMatch &    &          59.6 &  58.3 &  59.6 &    &         60.8 &  59.3 &  60.9 &    &        61.3 &  60.4 &  62.5 &    &        62.0 &  63.6 &  66.6 &    &        58.1 &  62.2 &  65.5 \\
      RS-FixMatch &    &          57.6 &  56.2 &  57.5 &    &         58.3 &  57.5 &  58.7 &    &        57.8 &  57.0 &  59.3 &    &        59.0 &  59.2 &  64.4 &    &        54.7 &  59.0 &  63.2 \\
     NoisyStudent &    &          61.5 &  60.3 &  61.5 &    &         62.1 &  60.5 &  62.1 &    &        60.5 &  60.3 &  61.7 &    &        61.8 &  62.5 &  66.0 &    &        57.2 &  61.5 &  64.9 \\
  RS-NoisyStudent &    &          61.2 &  59.7 &  61.1 &    &         61.7 &  60.0 &  61.8 &    &        61.3 &  60.6 &  62.3 &    &        61.2 &  62.0 &  66.4 &    &        59.5 &  63.3 &  66.3 \\
           SENTRY &    &          51.4 &  46.0 &  51.3 &    &         51.7 &  47.4 &  52.0 &    &        50.0 &  45.5 &  51.7 &    &        50.0 &  46.6 &  55.9 &    &        45.0 &  44.1 &  55.6 \\
 \bottomrule
 \end{tabular}
 
 

==> tables/living17.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
Source (w/o aug) &    &          66.3 &  65.4 &  66.3 &    &         68.9 &  68.8 &  68.9 &    &        69.8 &  69.8 &  72.3 &    &        66.0 &  68.9 &  76.9 &    &        64.8 &  66.9 &  88.6 \\
  Source (w aug) &    &          72.8 &  71.6 &  72.8 &    &         75.8 &  74.2 &  75.9 &    &        76.1 &  74.0 &  75.5 &    &        71.5 &  72.5 &  81.1 &    &        76.3 &  78.9 &  86.5 \\
    Source (adv) &    &          51.7 &  45.3 &  51.7 &    &         52.5 &  47.7 &  55.1 &    &        50.8 &  48.1 &  57.3 &    &        50.6 &  50.0 &  66.3 &    &        40.8 &  57.8 &  80.8 \\
   Source (clip) &    &          90.0 &  89.9 &  90.0 &    &         92.9 &  92.8 &  93.0 &    &        93.9 &  93.9 &  94.2 &    &        91.9 &  92.0 &  94.7 &    &        96.4 &  97.6 &  98.0 \\
            DARE &    &          66.6 &  66.2 &  66.6 &    &         66.2 &  66.2 &  66.3 &    &        59.8 &  58.9 &  61.3 &    &        43.8 &  44.2 &  57.0 &    &        29.1 &  31.4 &  54.8 \\
        BN-adapt &    &          73.4 &  72.7 &  73.4 &    &         75.4 &  74.0 &  75.5 &    &        74.2 &  73.4 &  74.0 &    &        69.3 &  70.7 &  79.5 &    &        65.6 &  69.5 &  85.0 \\
     RS-BN-adapt &    &          72.4 &  72.0 &  72.4 &    &         75.2 &  73.8 &  75.4 &    &        74.5 &  74.6 &  73.9 &    &        70.7 &  72.2 &  80.6 &    &        62.8 &  72.1 &  86.3 \\
            TENT &    &          72.2 &  71.8 &  72.2 &    &         74.4 &  73.7 &  74.6 &    &        74.3 &  73.5 &  74.0 &    &        69.4 &  70.9 &  79.5 &    &        65.6 &  69.3 &  85.0 \\
         RS-TENT &    &          72.4 &  72.0 &  72.4 &    &         75.2 &  73.8 &  75.4 &    &        74.5 &  74.6 &  73.9 &    &        70.7 &  72.2 &  80.6 &    &        62.8 &  72.1 &  86.3 \\
            DANN &    &          69.7 &  68.2 &  69.7 &    &         72.1 &  71.4 &  73.1 &    &        73.1 &  73.3 &  74.8 &    &        72.8 &  73.7 &  79.9 &    &        54.8 &  70.1 &  85.5 \\
         IW-DANN &    &          68.6 &       &       &    &         74.4 &       &       &    &        72.9 &       &       &    &        72.2 &       &       &    &        71.9 &       &       \\
         RS-DANN &    &          68.7 &  67.9 &  68.7 &    &         70.0 &  70.0 &  70.3 &    &        72.3 &  71.4 &  71.8 &    &        74.6 &  77.8 &  81.8 &    &        66.9 &  70.6 &  84.7 \\
           CDANN &    &          68.5 &  68.0 &  68.5 &    &         70.2 &  70.1 &  71.1 &    &        72.7 &  71.5 &  75.2 &    &        72.3 &  73.4 &  77.3 &    &        67.4 &  76.5 &  91.7 \\
        IW-CDANN &    &          70.7 &       &       &    &         71.5 &       &       &    &        76.2 &       &       &    &        70.2 &       &       &    &        61.0 &       &       \\
        RS-CDANN &    &          71.6 &  70.5 &  71.6 &    &         73.6 &  72.9 &  73.8 &    &        71.4 &  69.4 &  74.1 &    &        72.0 &  72.7 &  83.4 &    &        67.5 &  76.8 &  85.1 \\
        FixMatch &    &          76.2 &  76.3 &  76.2 &    &         77.0 &  76.3 &  77.8 &    &        78.2 &  78.2 &  80.5 &    &        78.1 &  79.1 &  87.0 &    &        66.0 &  69.3 &  84.9 \\
     RS-FixMatch &    &          74.2 &  74.2 &  74.2 &    &         78.4 &  78.3 &  79.0 &    &        78.2 &  78.2 &  79.5 &    &        80.2 &  83.2 &  86.2 &    &        67.9 &  70.6 &  86.3 \\
    NoisyStudent &    &          70.5 &  71.4 &  70.5 &    &         77.1 &  76.4 &  77.3 &    &        76.5 &  74.3 &  75.9 &    &        77.4 &  75.4 &  83.4 &    &        71.5 &  73.8 &  87.4 \\
 RS-NoisyStudent &    &          73.0 &  71.6 &  73.0 &    &         77.3 &  77.1 &  77.3 &    &        75.2 &  76.1 &  77.6 &    &        70.5 &  75.2 &  87.9 &    &        58.9 &  79.2 &  87.2 \\
          SENTRY &    &          65.5 &  64.4 &  65.5 &    &         65.4 &  62.6 &  65.6 &    &        48.9 &  49.0 &  48.1 &    &        48.3 &  48.8 &  63.2 &    &        43.5 &  40.4 &  75.9 \\
\bottomrule
\end{tabular}


==> tables/nonliving26.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
Source (w/o aug) &    &          54.1 &  54.0 &  54.1 &    &         53.2 &  52.5 &  52.7 &    &        54.3 &  53.6 &  54.7 &    &        62.5 &  62.8 &  67.2 &    &        49.5 &  51.6 &  65.5 \\
  Source (w aug) &    &          62.7 &  61.9 &  62.7 &    &         62.6 &  61.7 &  62.2 &    &        60.9 &  60.3 &  63.7 &    &        62.3 &  65.9 &  71.5 &    &        59.0 &  64.1 &  72.4 \\
    Source (adv) &    &          55.8 &  53.2 &  55.8 &    &         54.0 &  50.2 &  55.1 &    &        56.2 &  53.0 &  56.7 &    &        58.4 &  61.2 &  66.7 &    &        46.5 &  51.7 &  61.2 \\
   Source (clip) &    &          82.4 &  82.5 &  82.4 &    &         84.4 &  84.4 &  84.5 &    &        86.6 &  85.9 &  88.4 &    &        83.3 &  81.9 &  88.6 &    &        85.7 &  86.3 &  91.6 \\
            DARE &    &          55.8 &  55.3 &  55.8 &    &         57.2 &  57.6 &  57.2 &    &        51.7 &  52.7 &  54.6 &    &        41.9 &  42.2 &  60.9 &    &        19.4 &  20.6 &  44.4 \\
        BN-adapt &    &          62.4 &  62.1 &  62.4 &    &         62.0 &  61.2 &  61.9 &    &        60.0 &  59.8 &  63.2 &    &        61.0 &  65.1 &  71.0 &    &        55.9 &  62.2 &  71.4 \\
     RS-BN-adapt &    &          62.5 &  62.1 &  62.5 &    &         62.7 &  61.3 &  62.4 &    &        60.3 &  59.7 &  63.2 &    &        63.2 &  65.7 &  69.8 &    &        60.7 &  63.0 &  72.1 \\
            TENT &    &          62.6 &  62.3 &  62.6 &    &         62.0 &  61.2 &  61.9 &    &        60.0 &  59.8 &  63.2 &    &        61.0 &  65.1 &  71.0 &    &        55.9 &  62.2 &  71.4 \\
         RS-TENT &    &          62.5 &  62.2 &  62.5 &    &         62.7 &  61.4 &  62.4 &    &        60.3 &  59.8 &  63.2 &    &        63.2 &  65.7 &  69.8 &    &        60.7 &  63.0 &  72.1 \\
            DANN &    &          59.6 &  59.0 &  59.5 &    &         59.2 &  57.2 &  58.4 &    &        55.6 &  57.6 &  57.8 &    &        62.4 &  64.3 &  70.3 &    &        59.7 &  65.4 &  74.2 \\
         IW-DANN &    &          59.6 &       &       &    &         61.2 &       &       &    &        60.3 &       &       &    &        62.3 &       &       &    &        56.4 &       &       \\
         RS-DANN &    &          57.9 &  57.5 &  57.9 &    &         56.1 &  55.5 &  56.2 &    &        58.6 &  57.8 &  58.2 &    &        57.3 &  57.6 &  69.8 &    &        53.6 &  54.4 &  73.9 \\
           CDANN &    &          58.0 &  57.2 &  58.0 &    &         57.4 &  57.0 &  58.1 &    &        59.4 &  58.8 &  61.6 &    &        55.8 &  60.2 &  67.6 &    &        50.6 &  56.9 &  70.7 \\
        IW-CDANN &    &          59.6 &       &       &    &         57.5 &       &       &    &        57.8 &       &       &    &        61.8 &       &       &    &        56.6 &       &       \\
        RS-CDANN &    &          59.9 &  58.4 &  59.9 &    &         57.5 &  58.0 &  57.6 &    &        59.4 &  61.4 &  60.9 &    &        59.9 &  59.7 &  68.7 &    &        56.9 &  62.6 &  74.2 \\
        FixMatch &    &          66.2 &  65.4 &  66.2 &    &         64.8 &  62.9 &  66.4 &    &        62.4 &  63.6 &  66.1 &    &        64.9 &  64.1 &  75.7 &    &        52.7 &  53.3 &  81.3 \\
     RS-FixMatch &    &          64.6 &  62.8 &  64.6 &    &         67.5 &  66.9 &  67.5 &    &        64.7 &  64.0 &  64.1 &    &        61.3 &  61.8 &  72.0 &    &        56.2 &  61.3 &  73.9 \\
    NoisyStudent &    &          64.2 &  63.1 &  64.1 &    &         61.8 &  63.0 &  62.7 &    &        60.0 &  59.4 &  61.9 &    &        66.4 &  67.0 &  72.3 &    &        57.1 &  59.1 &  75.5 \\
 RS-NoisyStudent &    &          62.1 &  61.9 &  62.1 &    &         63.2 &  61.3 &  63.4 &    &        59.9 &  60.7 &  62.6 &    &        65.9 &  67.6 &  74.8 &    &        62.2 &  64.8 &  75.8 \\
          SENTRY &    &          55.9 &  54.1 &  55.9 &    &         41.2 &  35.5 &  42.5 &    &        46.4 &  42.1 &  48.5 &    &        39.5 &  38.7 &  49.0 &    &        24.5 &  24.4 &  58.7 \\
\bottomrule
\end{tabular}


==> tables/officehome.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
 Source (w/o aug) &    &          62.6 &  58.5 &  62.7 &    &         63.7 &  60.3 &  64.3 &    &        65.0 &  61.1 &  65.8 &    &        66.4 &  67.2 &  73.1 &    &        62.0 &  63.0 &  73.4 \\
   Source (w aug) &    &          62.2 &  59.2 &  62.0 &    &         63.3 &  59.7 &  64.5 &    &        64.5 &  62.4 &  66.5 &    &        66.5 &  68.9 &  72.1 &    &        66.4 &  66.4 &  73.4 \\
     Source (adv) &    &          56.5 &  50.9 &  56.3 &    &         58.5 &  52.6 &  59.6 &    &        59.5 &  55.5 &  60.7 &    &        60.7 &  61.3 &  70.5 &    &        60.1 &  54.5 &  72.1 \\
    Source (clip) &    &          79.8 &  77.3 &  80.2 &    &         79.2 &  77.5 &  79.9 &    &        78.9 &  77.5 &  80.2 &    &        79.4 &  78.7 &  83.9 &    &        78.5 &  79.3 &  88.0 \\
             DARE &    &          59.4 &  59.2 &  60.6 &    &         56.5 &  56.4 &  59.2 &    &        53.1 &  52.4 &  58.1 &    &        39.6 &  37.9 &  56.7 &    &        32.6 &  32.9 &  59.7 \\
         BN-adapt &    &          62.8 &  61.3 &  64.9 &    &         65.0 &  64.1 &  66.4 &    &        66.4 &  64.8 &  69.1 &    &        67.0 &  69.2 &  75.5 &    &        67.2 &  68.2 &  76.2 \\
      RS-BN-adapt &    &          63.2 &  60.9 &  64.1 &    &         65.3 &  62.8 &  66.0 &    &        66.9 &  63.3 &  68.7 &    &        67.6 &  68.7 &  74.3 &    &        66.7 &  67.7 &  76.2 \\
             TENT &    &          62.8 &  61.6 &  64.8 &    &         65.1 &  63.7 &  66.0 &    &        66.0 &  65.3 &  68.8 &    &        67.3 &  69.2 &  74.9 &    &        66.7 &  68.9 &  75.4 \\
          RS-TENT &    &          63.2 &  61.0 &  64.1 &    &         65.1 &  62.9 &  66.2 &    &        66.9 &  63.4 &  68.8 &    &        67.3 &  69.4 &  74.3 &    &        66.7 &  67.9 &  76.2 \\
             DANN &    &          66.6 &  65.1 &  67.5 &    &         67.2 &  65.6 &  67.8 &    &        67.7 &  67.7 &  69.4 &    &        68.3 &  70.2 &  77.2 &    &        62.9 &  64.7 &  75.2 \\
          IW-DANN &    &          66.9 &       &       &    &         67.6 &       &       &    &        67.7 &       &       &    &        67.7 &       &       &    &        63.1 &       &       \\
          RS-DANN &    &          67.5 &  65.3 &  68.0 &    &         67.1 &  65.4 &  68.0 &    &        67.6 &  65.0 &  69.4 &    &        70.7 &  70.1 &  76.6 &    &        65.4 &  67.4 &  75.4 \\
            CDANN &    &          66.3 &  65.0 &  66.9 &    &         66.5 &  65.8 &  67.7 &    &        66.9 &  65.6 &  68.7 &    &        68.7 &  70.8 &  77.9 &    &        63.9 &  65.7 &  75.5 \\
         IW-CDANN &    &          66.3 &       &       &    &         66.6 &       &       &    &        66.7 &       &       &    &        68.6 &       &       &    &        63.4 &       &       \\
         RS-CDANN &    &          65.2 &  63.5 &  65.9 &    &         66.9 &  65.1 &  66.8 &    &        67.6 &  65.1 &  67.0 &    &        65.7 &  66.3 &  75.1 &    &        63.2 &  61.0 &  75.2 \\
         FixMatch &    &          62.5 &  57.9 &  62.5 &    &         64.1 &  58.7 &  63.9 &    &        65.9 &  60.9 &  65.1 &    &        65.2 &  66.9 &  72.9 &    &        66.2 &  67.4 &  75.9 \\
      RS-FixMatch &    &          62.9 &  57.1 &  61.5 &    &         63.4 &  57.8 &  62.9 &    &        65.3 &  58.3 &  64.8 &    &        68.9 &  66.4 &  72.7 &    &        62.4 &  63.4 &  72.1 \\
     NoisyStudent &    &          65.0 &  61.3 &  65.2 &    &         65.6 &  63.1 &  66.4 &    &        67.0 &  65.5 &  68.1 &    &        69.9 &  68.0 &  75.6 &    &        66.3 &  65.6 &  76.7 \\
  RS-NoisyStudent &    &          65.3 &  62.0 &  64.9 &    &         65.4 &  62.8 &  66.1 &    &        67.3 &  65.3 &  67.6 &    &        70.4 &  68.4 &  75.8 &    &        65.8 &  65.8 &  76.2 \\
           SENTRY &    &          58.1 &  53.1 &  57.9 &    &         58.4 &  52.7 &  59.6 &    &        59.8 &  55.4 &  61.1 &    &        62.1 &  61.3 &  68.8 &    &        54.1 &  53.8 &  68.0 \\
 \bottomrule
 \end{tabular}
 
 

==> tables/visda.tex <==
\begin{tabular}{llccccccccccccccccccc}
    \toprule
                   & & \multicolumn{3}{c}{Alpha = \textsc{None}} &  & \multicolumn{3}{c}{Alpha = 10.0} & & \multicolumn{3}{c}{Alpha = 3.0} & & \multicolumn{3}{c}{Alpha = 1.0} &  & \multicolumn{3}{c}{Alpha = 0.5} \\
 Algorithm &  &         {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &        {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True} &  &     {\scriptsize None} & {\scriptsize RLLS} & {\scriptsize True}  \\
 \midrule
 Source (w/o aug) &    &          64.0 &  60.4 &  63.7 &    &         62.8 &  59.6 &  63.6 &    &        61.7 &  58.9 &  63.9 &    &        57.5 &  56.2 &  62.4 &    &        65.8 &  67.6 &  75.8 \\
   Source (w aug) &    &          60.8 &  57.9 &  60.6 &    &         59.2 &  56.5 &  59.8 &    &        57.7 &  55.3 &  59.2 &    &        55.7 &  54.1 &  58.0 &    &        65.4 &  66.3 &  73.3 \\
     Source (adv) &    &          57.3 &  54.2 &  57.0 &    &         55.6 &  52.7 &  56.0 &    &        54.0 &  51.3 &  55.0 &    &        51.6 &  49.8 &  53.9 &    &        60.1 &  59.7 &  70.0 \\
    Source (clip) &    &          75.5 &  73.2 &  75.5 &    &         74.8 &  72.8 &  75.7 &    &        74.2 &  72.5 &  76.1 &    &        73.1 &  72.7 &  76.7 &    &        78.2 &  79.6 &  82.1 \\
             DARE &    &          63.3 &  63.2 &  63.7 &    &         61.7 &  61.7 &  62.7 &    &        60.3 &  60.4 &  62.0 &    &        57.4 &  57.8 &  60.7 &    &        52.0 &  54.9 &  63.5 \\
         BN-adapt &    &          71.5 &  71.3 &  72.3 &    &         71.4 &  71.4 &  73.2 &    &        69.9 &  70.1 &  73.0 &    &        65.9 &  67.3 &  73.3 &    &        57.1 &  63.2 &  74.5 \\
      RS-BN-adapt &    &          70.1 &  68.8 &  70.4 &    &         69.3 &  68.5 &  70.6 &    &        67.6 &  67.0 &  69.8 &    &        64.1 &  63.5 &  68.2 &    &        67.8 &  71.0 &  76.8 \\
             TENT &    &          73.6 &  73.6 &  74.5 &    &         72.5 &  72.5 &  74.2 &    &        70.9 &  71.3 &  74.0 &    &        66.6 &  67.4 &  73.4 &    &        58.5 &  64.5 &  74.7 \\
          RS-TENT &    &          71.7 &  70.7 &  72.0 &    &         70.7 &  70.2 &  71.9 &    &        68.4 &  68.0 &  70.7 &    &        64.4 &  63.9 &  68.3 &    &        68.2 &  71.3 &  76.9 \\
             DANN &    &          76.0 &  75.9 &  76.3 &    &         73.8 &  73.9 &  74.4 &    &        72.4 &  72.6 &  73.6 &    &        64.9 &  65.0 &  66.8 &    &        54.0 &  54.3 &  60.3 \\
          IW-DANN &    &          77.0 &       &       &    &         73.5 &       &       &    &        71.7 &       &       &    &        64.0 &       &       &    &        53.6 &       &       \\
          RS-DANN &    &          77.5 &  77.4 &  77.6 &    &         76.8 &  76.8 &  77.3 &    &        77.0 &  77.3 &  78.3 &    &        68.9 &  68.8 &  70.8 &    &        59.3 &  60.2 &  66.5 \\
            CDANN &    &          80.3 &  80.3 &  80.4 &    &         78.1 &  78.2 &  78.4 &    &        74.4 &  74.5 &  75.1 &    &        64.6 &  64.4 &  65.8 &    &        57.8 &  58.1 &  60.2 \\
         IW-CDANN &    &          79.4 &       &       &    &         78.5 &       &       &    &        74.5 &       &       &    &        64.4 &       &       &    &        56.4 &       &       \\
         RS-CDANN &    &          79.7 &  79.6 &  79.7 &    &         76.7 &  76.6 &  76.9 &    &        79.8 &  79.9 &  80.4 &    &        71.4 &  71.0 &  72.4 &    &        64.1 &  64.4 &  66.4 \\
         FixMatch &    &          80.7 &  80.7 &  81.4 &    &         77.5 &  77.3 &  78.7 &    &        75.9 &  75.8 &  78.5 &    &        73.1 &  73.6 &  78.8 &    &        60.3 &  63.5 &  71.9 \\
      RS-FixMatch &    &          80.8 &  80.7 &  81.2 &    &         80.7 &  80.5 &  81.4 &    &        79.7 &  79.6 &  82.0 &    &        72.9 &  72.7 &  77.7 &    &        72.3 &  74.9 &  79.9 \\
     NoisyStudent &    &          62.6 &  59.8 &  62.6 &    &         60.1 &  57.7 &  60.8 &    &        59.0 &  56.9 &  60.3 &    &        57.5 &  57.0 &  58.8 &    &        66.3 &  67.2 &  72.4 \\
  RS-NoisyStudent &    &          62.3 &  59.7 &  62.4 &    &         60.6 &  58.0 &  61.1 &    &        58.4 &  56.2 &  60.0 &    &        57.1 &  56.1 &  58.1 &    &        67.8 &  68.6 &  73.9 \\
           SENTRY &    &          78.3 &  77.9 &  78.6 &    &         81.3 &  81.0 &  81.9 &    &        79.8 &  79.0 &  81.4 &    &        72.2 &  72.7 &  73.9 &    &        74.5 &  76.8 &  80.8 \\
 \bottomrule
 \end{tabular}
 
